Coordination via Interaction Constraints I: Local Logic

Wegner describes coordination as constrained interaction. We take this approach literally and define a coordination model based on interaction constraints and partial, iterative and interactive constraint satisfaction. Our model captures behaviour described in terms of synchronisation and data flow constraints, plus various modes of interaction with the outside world provided by external constraint symbols, on-the-fly constraint generation, and coordination variables. Underlying our approach is an engine performing (partial) constraint satisfaction of the sets of constraints. Our model extends previous work on three counts: firstly, a more advanced notion of external interaction is offered; secondly, our approach enables local satisfaction of constraints with appropriate partial solutions, avoiding global synchronisation over the entire constraints set; and, as a consequence, constraint satisfaction can finally occur concurrently, and multiple parts of a set of constraints can be solved and interact with the outside world in an asynchronous manner, unless synchronisation is required by the constraints. This paper describes the underlying logic, which enables a notion of local solution, and relates this logic to the more global approach of our previous work based on classical logic.

==> eptcsdata.tex <==
\providecommand{\event}{F. Bonchi, D. Grohmann, P. Spoletini, and E. Tuosto:\\ 
   ICE'09 Structured Interactions}
\providecommand{\volume}{12}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{17}
\providecommand{\eid}{2}
\pdfoutput=1

